Privacy-Preserving Group Data Access via Stateless Oblivious RAM Simulation

We study the problem of providing privacy-preserving access to an outsourced honest-but-curious data repository for a group of trusted users. We show that such privacy-preserving data access is possible using a combination of probabilistic encryption, which directly hides data values, and stateless oblivious RAM simulation, which hides the pattern of data accesses. We give simulations that have only an $O(\log n)$ amortized time overhead for simulating a RAM algorithm, $\cal A$, that has a memory of size $n$, using a scheme that is data-oblivious with very high probability assuming the simulation has access to a private workspace of size $O(n^\nu)$, for any given fixed constant $\nu>0$. This simulation makes use of pseudorandom hash functions and is based on a novel hierarchy of cuckoo hash tables that all share a common stash. We also provide results from an experimental simulation of this scheme, showing its practicality. In addition, in a result that may be of some theoretical interest, we also show that one can eliminate the dependence on pseudorandom hash functions in our simulation while having the overhead rise to be $O(\log^2 n)$.

==> sharedstash.tex <==
\section{Shared-Stash Cuckoo Hashing}
\label{sec:sharedstash}

We claim that, given our recursive construction, we require a total
stash size of only $O(\log n)$.  That is, if we consider the sum of
the number of items placed in the stash at all possible levels in our
construction, this will be at most $O(\log n)$ with high probability.  

The key is the following argument.  As shown
in \cite{gm-paodor-11}, at a level of size $m$ cells where $m$
is $\Omega(log^7 n)$, the probability that the stash for that level
exceeds a total size $s$ is $m^{-\Omega(s)}$.  Further, as long as the
hashes for each level in our construction are independent, we can
treat the required stash size at each level is independent, since the
number of items placed in the stash at a level is then a random
variable dependent only on the number of items appearing in that
level.

Now consider any point of our construction and let $S_i$ be the
number of items at the $i$th level that need to be put in the stash.
It is apparent that $S_i$ has mean less than 1 and tails that can be
dominated by a geometrically decreasing random variable.  This is
sufficient to apply standard Chernoff bounds.  Formally, let $X_1,
X_2, \ldots, X_\ell$ be independent random variables with mean 1
geometrically decreasing tails, so that $X_i = j$ with probability
$1/2^{j}$ for $j \geq 1$.  Then the calculations
of \cite{gm-paodor-11} imply that the $X_i$ stochastically
dominate the $S_i$, and we can now apply standard Chernoff bounds for
these random variables.  Specifically, noting that $X_i$ can be
interpreted as the number of fair coin flips until the first heads, we
can think of the sum of the $X_i$ as being the number of coin flips
until the $\ell$th head, and this dominates the number of items that
need to be placed in the stash at any point.  When $\ell = O(\log n)$,
as is the case here as there are only $O(\log n)$ levels of hash
tables in our construction, then for any constant $\gamma$ there
exists a corresponding constant $\nu$ such that the $\ell$th head
occurs by the $(\nu \log n)$'th flip with probability at least
$1-1/n^\gamma$.  Hence we can handle any polynomial number of steps
with high probability, using a stash of size only $O(\log n)$ that
holds items from all levels of our construction.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

